Human Factors in Security Research: Lessons Learned from 2008-2018

Instead of only considering technology, computer security research now strives to also take into account the human factor by studying regular users and, to a lesser extent, experts like operators and developers of systems. We focus our analysis on the research on the crucial population of experts, whose human errors can impact many systems at once, and compare it to research on regular users. To understand how far we advanced in the area of human factors, how the field can further mature, and to provide a point of reference for researchers new to this field, we analyzed the past decade of human factors research in security and privacy, identifying 557 relevant publications. Of these, we found 48 publications focused on expert users and analyzed all in depth. For additional insights, we compare them to a stratified sample of 48 end-user studies. In this paper we investigate: (i) The perspective on human factors, and how we can learn from safety science (ii) How and who are the participants recruited, and how this -- as we find -- creates a western-centric perspective (iii) Research objectives, and how to align these with the chosen research methods (iv) How theories can be used to increase rigor in the communities scientific work, including limitations to the use of Grounded Theory, which is often incompletely applied (v) How researchers handle ethical implications, and what we can do to account for them more consistently Although our literature review has limitations, new insights were revealed and avenues for further research identified.

==> human-factors.tex <==




\begin{figure*}[t!]
\centering
\includegraphics[width=1\textwidth]{figures/safety_timeline.pdf}

%\resizebox{\textwidth}{!}{
%\begin{tikzpicture}[]
%\MyDesc{1900's}{Taylorism\textsuperscript{\cite{taylor1911, dekker2016, Addingtoolbox, dekker2019foundations, swuste2010safety, Hollnagel2013}}\\Accident Proneness\textsuperscript{\cite{dekker2019foundations, swuste2010safety, burnham2010accident}}\\Newtonian view\textsuperscript{\cite{dekker2016, dekker2010system}} \begin{itemize} \item \footnotesize Description: \begin{itemize} \item Accidents have preventable causes \item Certain people are prone to accidents \item Time-motion studies \item Proceduralization and violations  \item[] ~ \\ ~ \end{itemize} \item Level of analysis\textsuperscript{\cite{van1999risks}}: \begin{itemize} \item Individual \item[] ~ \item[] ~ \end{itemize}\end{itemize}}
%\MyDesc[right = 8.1cm of desc1.west]{1930's}{Heinrich domino model\textsuperscript{\cite{swuste2010safety, Hollnagel2013}}\\Heinrich iceberg model\textsuperscript{\cite{swuste2010safety}}\\Behavior based safety\textsuperscript{\cite{dekker2019foundations, frederick2000blame}} \begin{itemize}\item \footnotesize Description: \begin{itemize} \item Cause \& effect are linear \item Decomposable systems \item Bimodal functionality \item Compliance \item Human error \\ ~\end{itemize} \item Level of analysis\textsuperscript{\cite{van1999risks}}: \begin{itemize} \item Individual  \item[] ~ \item[] ~ \end{itemize}\end{itemize}}
%\MyDesc[right = 8.1cm of desc2.west]{1950's}{Systems thinking\textsuperscript{\cite{Addingtoolbox, dekker2019foundations}}\\Human Factors\textsuperscript{\cite{dekker2019foundations, adams2006layman}}\\Gibson-Haddon's work\textsuperscript{\cite{guarnieri1992landmarks}}\begin{itemize}\item \footnotesize Description: \begin{itemize} \item Complex systems theory \item Not \underline{who} but \underline{what} is responsible \item Ergonomics \item Shift from psychology to engineering and epidemiology \item Proceduralization and violations \end{itemize} \item Level of analysis\textsuperscript{\cite{van1999risks}}: \begin{itemize} \item Individual \item Organizational  \item[] ~  \end{itemize}\end{itemize}}
%\MyDesc[right = 8.1cm of desc3.west]{1970's}{ Swiss cheese model\textsuperscript{\cite{dekker2016, Addingtoolbox, dekker2019foundations, reason1998achieving}}\\Normal accident theory\textsuperscript{\cite{dekker2019foundations, perrow1984normal}}\\High-reliability organizations\textsuperscript{\cite{dekker2019foundations, weick1987organizational}} \begin{itemize} \item \footnotesize Description: \begin{itemize} \item Latent conditions behind failure \item Judgement and bureaucracy \item Organizational culture \item Loose vs. tight coupling  \item[] ~ \\ ~ \end{itemize} \item Level of analysis\textsuperscript{\cite{van1999risks}}: \begin{itemize} \item Individual \item Organizational  \item[] ~  \end{itemize}\end{itemize}}
%\MyDesc[right = 8.1cm of desc4.west]{2000's}{ Safety II\textsuperscript{\cite{Hollnagel2013}}\\Resilience\textsuperscript{\cite{dekker2016, dekker2019foundations, Hollnagel2013, dekker2008resilience}}\\Restorative justice\textsuperscript{\cite{dekker2018just}} \begin{itemize}\item \footnotesize Description: \begin{itemize} \item Emergence of success and failure \item Variable performance \item How do things go well? \item No-blame culture \item Trust and accountability \\ ~ \end{itemize} \item Level of analysis\textsuperscript{\cite{van1999risks}}: \begin{itemize} \item Individual \item Organizational \item Societal\end{itemize}\end{itemize}}
%\node[myshape,right = 6.5cm of desc5.west] {NOW};
%\end{tikzpicture}
%
%}
%


\caption{Overview of the development of human factors research in safety science~\cite{dekker2019foundations}. Note how over time, the perspective shifted away from individual responsibility to, first, organizational factors, and finally to a societal perspective.
%\mve{would institutional not be a more accurate description than societal?}
%\tf{Institutional/organizational is the first step in bobble4; In the last step, also societal factors are considered, i.e., how we consider responsibility etc.}
Ultimately, the focus is no longer on how to prevent human error, but instead, on how to facilitate proper resilient operations.
\nocite{taylor1911, dekker2016, Addingtoolbox, dekker2019foundations, swuste2010safety, Hollnagel2013, dekker2019foundations, swuste2010safety, burnham2010accident, dekker2016, dekker2010system, van1999risks, swuste2010safety, Hollnagel2013, swuste2010safety, dekker2019foundations, frederick2000blame, Addingtoolbox, dekker2019foundations, dekker2019foundations, adams2006layman, guarnieri1992landmarks, dekker2016, Addingtoolbox, dekker2019foundations, reason1998achieving, dekker2019foundations, perrow1984normal, dekker2019foundations, weick1987organizational, Hollnagel2013, dekker2016, dekker2019foundations, Hollnagel2013, dekker2008resilience, dekker2018just}
%
}
\label{fig:hf-stages}
\end{figure*}


%% Uncomment this to get the proper reference numbers for figure 2
%\begin{itemize}
%\item next
%\item 1.1 \cite{taylor1911, dekker2016, Addingtoolbox, dekker2019foundations, swuste2010safety, Hollnagel2013}
%\item 1.2 \cite{dekker2019foundations, swuste2010safety, burnham2010accident}
%\item 1.3 \cite{dekker2016, dekker2010system}
%\item 1.4 \cite{van1999risks}
%%
%\item next
%\item 2.1 \cite{swuste2010safety, Hollnagel2013}
%\item 2.2 \cite{swuste2010safety}
%\item 2.3 \cite{dekker2019foundations, frederick2000blame}
%%
%\item next
%\item 3.1 \cite{Addingtoolbox, dekker2019foundations}
%\item 3.2 \cite{dekker2019foundations, adams2006layman}
%\item 3.3 \cite{guarnieri1992landmarks}
%%
%\item next
%\item 4.1 \cite{dekker2016, Addingtoolbox, dekker2019foundations, reason1998achieving}
%\item 4.2 \cite{dekker2019foundations, perrow1984normal}
%\item 4.3 \cite{dekker2019foundations, weick1987organizational}
%\item next
%\item 5.1 \cite{Hollnagel2013}
%\item 5.2 \cite{dekker2016, dekker2019foundations, Hollnagel2013, dekker2008resilience}
%\item 5.3 \cite{dekker2018just}
%\end{itemize}

